BEVFusion: Multi-Task Multi-Sensor Fusion with Unified Bird's-Eye View Representation

Multi-sensor fusion is essential for an accurate and reliable autonomous driving system. Recent approaches are based on point-level fusion: augmenting the LiDAR point cloud with camera features. However, the camera-to-LiDAR projection throws away the semantic density of camera features, hindering the effectiveness of such methods, especially for semantic-oriented tasks (such as 3D scene segmentation). In this paper, we break this deeply-rooted convention with BEVFusion, an efficient and generic multi-task multi-sensor fusion framework. It unifies multi-modal features in the shared bird's-eye view (BEV) representation space, which nicely preserves both geometric and semantic information. To achieve this, we diagnose and lift key efficiency bottlenecks in the view transformation with optimized BEV pooling, reducing latency by more than 40x. BEVFusion is fundamentally task-agnostic and seamlessly supports different 3D perception tasks with almost no architectural changes. It establishes the new state of the art on nuScenes, achieving 1.3% higher mAP and NDS on 3D object detection and 13.6% higher mIoU on BEV map segmentation, with 1.9x lower computation cost. Code to reproduce our results is available at https://github.com/mit-han-lab/bevfusion.

==> visuals/results/ablations.tex <==
\begin{table*}[t]
\centering
\caption{Ablation experiments to validate our design choices. Default settings are marked in \colorbox{gray!15}{gray}.}
\vspace{-5pt}
\label{tab:results:ablations}
\begin{subtable}[t]{0.27\linewidth}
\centering\small
\addtolength{\tabcolsep}{1pt} 
\caption{Modality}
\vspace{-5pt}
\scalebox{0.85}{
\begin{tabular}{cccc} \toprule
 & mAP & NDS & mIoU \\\midrule
L & 57.6 & 64.9 & 48.6 \\
C & 33.3 & 40.2 & 56.6 \\
L+C & \cellcolor{gray!15}\textbf{66.4} & \cellcolor{gray!15}\textbf{69.5} & \cellcolor{gray!15}\textbf{62.7} \\
\bottomrule 
\end{tabular}
}
\label{tab:results:ablations:baselines}
\end{subtable}
~~
\begin{subtable}[t]{0.27\linewidth}
\centering\small
\setlength{\tabcolsep}{6.2pt}
\vspace{0pt}
\caption{Data augmentation}
\vspace{-5pt}
\scalebox{0.85}{
\begin{tabular}{cccc}\toprule
 & mAP & NDS & mIoU \\
\midrule 
Image & 63.8 & 68.1 & 62.3 \\
LiDAR & 65.7 & 69.1 & 61.3 \\
Both & \cellcolor{gray!15}\textbf{66.4} & \cellcolor{gray!15}\textbf{69.5} & \cellcolor{gray!15}\textbf{62.7} \\
\bottomrule
\end{tabular}
}
\label{tab:results:ablations:augmentations}
\end{subtable}
~
\begin{subtable}[t]{0.37\linewidth}
\centering\small
\setlength{\tabcolsep}{5pt}
\vspace{0pt}
\caption{Image backbone}
\vspace{-5pt}
\scalebox{0.85}{
\begin{tabular}{cccc}\toprule
 & mAP & NDS & mIoU \\
\midrule 
ResNet50 & 65.3 & 68.9 & 59.2 \\
SwinT (freeze) & 66.1 & 69.3 & 52.8 \\
SwinT & \cellcolor{gray!15}\textbf{66.4} & \cellcolor{gray!15}\textbf{69.5} & \cellcolor{gray!15}\textbf{62.7} \\
\bottomrule
\end{tabular}
}
\label{tab:results:ablations:backbone}
\end{subtable}

\begin{subtable}[t]{0.27\linewidth}
\centering\small
\addtolength{\tabcolsep}{1pt} 
\vspace{3pt}
\caption{FPN size}
\vspace{-5pt}
\scalebox{0.85}{
\begin{tabular}{cccc}\toprule
 & mAP & NDS & mIoU \\
\midrule
1/16 & 66.2 & 69.4 & \textbf{62.7} \\
1/8 & \cellcolor{gray!15}\textbf{66.4} & \cellcolor{gray!15}\textbf{69.5} & \cellcolor{gray!15}\textbf{62.7} \\
1/4 & 66.0 & 69.2 & 58.8 \\
\bottomrule
\end{tabular}
}
\label{tab:results:ablations:fpn}
\end{subtable}
~~
\begin{subtable}[t]{0.27\linewidth}
\centering\small
\addtolength{\tabcolsep}{1pt} 
\vspace{3pt}
\caption{Voxel size}
\vspace{-5pt}
\scalebox{0.85}{
\begin{tabular}{cccc} \toprule
 & mAP & NDS & mIoU \\\midrule
0.075 & \textbf{67.1} & \textbf{70.2} & 60.6 \\
0.1 & \cellcolor{gray!15}66.4 & \cellcolor{gray!15}69.5 & \cellcolor{gray!15}62.7 \\
0.125 & 65.1 & 68.6 & \textbf{63.7} \\\bottomrule
\end{tabular}
}
\label{tab:results:ablations:voxel}
\end{subtable}
~
\begin{subtable}[t]{0.37\linewidth}
\centering\small
\addtolength{\tabcolsep}{1pt} 
\vspace{3pt}
\caption{Image size}
\vspace{-5pt}
\scalebox{0.85}{
\begin{tabular}{cccc}\toprule
 & mAP & NDS & mIoU \\
\midrule
128$\times$352 & 64.0 & 68.2 & 60.5 \\
256$\times$704 & \cellcolor{gray!15}66.4 & \cellcolor{gray!15}69.5 & \cellcolor{gray!15}\textbf{62.7} \\
384$\times$1056 & \textbf{67.2} & \textbf{70.0} & 59.9 \\
\bottomrule
\end{tabular}
}
\label{tab:results:ablations:image}
\end{subtable}
\vspace{-15pt}
\end{table*}

==> visuals/results/analysis_table_backup.tex <==
\begin{minipage}[t]{0.36\textwidth}
\centering\small
\addtolength{\tabcolsep}{1pt} 
\scalebox{0.82}{
\begin{tabular}{cccc} \toprule
   & mAP & NDS & mIoU \\\midrule
Det. only & 67.0 & 70.4 & -- \\
Seg. only & -- & -- & 58.5 \\
Joint (\textit{share}) & 65.5  & 69.7 & 54.0  \\
Joint (\textit{sep.}) & 65.9 & 69.9 & 58.4 \\
\bottomrule 
\end{tabular}
}
\captionof{table}{Joint training results}
\label{tab:results:analysis:joint}
\end{minipage}
\hfill
\begin{minipage}[t]{0.64\textwidth}
\centering\small
\addtolength{\tabcolsep}{1pt} 
\scalebox{0.82}{
\begin{tabular}{lcccc} \toprule
   & mAP (sunny) & mIoU (sunny) & mAP (rainy) & mIoU (rainy) \\\midrule
CenterPoint &  62.9 &  & 59.2 \\
MVP & 65.9 &  &  66.3 \\
\model-C & -- &  & -- & \\
\model & \textbf{68.2} &  & \textbf{69.9}  \\
\bottomrule 
\end{tabular}
}
\captionof{table}{Results under different weather.}
\label{tab:results:analysis:weather}
\end{minipage}

\begin{minipage}[t]{0.36\textwidth}
\centering\small
\addtolength{\tabcolsep}{1pt} 
\scalebox{0.82}{
\begin{tabular}{cccc} \toprule
   & 0-20m & 20-30m & >30m \\\midrule
SECOND & \\
MVP & \\
BEVFusion-C & \\
BEVFusion & \\
\bottomrule 
\end{tabular}
}
\captionof{table}{Seg. mIoU \vs distance.}
\label{tab:results:analysis:distances}
\end{minipage}
\hfill
\begin{minipage}[t]{0.64\textwidth}
\centering\small
\addtolength{\tabcolsep}{1pt} 
\scalebox{0.8}{
\begin{tabular}{lcccc} \toprule
   & mAP (day) & mIoU (day) & mAP (night) & mIoU (night)\\\midrule
CenterPoint & 62.8 &   & 35.4\\
MVP & 66.3 &  & 38.4 \\
\model-C & -- &  & -- & \\
\model & \textbf{68.5}  &  &  \textbf{42.8} \\
\bottomrule 
\end{tabular}
}
\captionof{table}{Results under different lighting conditions.}
\label{tab:results:analysis:lighting}
\end{minipage}



==> visuals/results/detection_test.tex <==
\begin{table*}[h]
\caption{Detailed metrics on the \texttt{test} split of nuScenes detection benchmark. \model achieves state-of-the-art results with 8.4 FPS inference speed on RTX 3090. Here, $\dag$ means test-time augmentation and $\ddag$ means test-time augmentation and model ensemble.}
\label{tab:results:detection:test}
\setlength{\tabcolsep}{2pt}
\small\centering 
\begin{tabular}{lccccccccccccc} \toprule
& Modality & mAP & NDS & Car & Truck & Bus & Trailer & C.V. & Ped. & Motor. & Bike & Cone & Barrier        \\\midrule
SECOND~\cite{yan2018second} & L & 52.8 & 63.3 & 81.1 & 48.5 & 54.9 & 42.9 & 10.5 & 80.1 & 51.5 & 22.3 & 70.9 & 65.7\\
CenterPoint~\cite{yin2021center} & L & 60.3 & 67.3 & 85.2 & 53.5 & 63.6 & 56.0 & 20.0 & 84.6 & 59.5 & 30.7 & 78.4 & 71.1\\
TransFusion-L~\cite{bai2022transfusion} & L & 65.5 & 70.2 & 86.2 & 56.7 & 66.3 & 58.8 & 28.2 & 86.1 & 68.3 & 44.2 & 82.0 & 78.2
\\\midrule
CenterPointV2~\cite{yin2021center}$\ddag$ & C+L+R & 67.1 & 71.4 & 87.0 & 57.3 & 69.3 & 60.4 & 28.8 & \textbf{90.4} & 71.3 & 49.0 & \textbf{86.8} & 71.0\\
PointAugmenting~\cite{wang2021pointaugmenting}$\dag$ & C+L & 66.8 & 71.1 & 87.5 & 57.3 & 65.2 & 60.7 & 28.0 & 87.9 & 74.3 & 50.9 & 83.6 & 72.6\\
MVP~\cite{yin2021multimodal} & C+L & 66.4 & 70.5 & 86.8 & 58.5 & 67.4 & 57.3 & 26.1 & 89.1 & 70.0 & 49.3 & 85.0 & 74.8\\
FusionPainting~\cite{xu2021fusionpainting} & C+L & 68.1 & 71.6 & 87.1 & \textbf{60.8} & 68.5 & 61.7 & 30.0 & 88.3 & \textbf{74.7} & \textbf{53.5} & 85.0 & 71.8 \\
AutoAlignV2~\cite{chen2022autoalign} & C+L & 68.4 & 72.4 & 87.0 & 59.0 & 69.3 & 59.3 & 33.1 & 87.6 & 72.9 & 52.1 & 85.1 & 78.0\\
TransFusion~\cite{bai2022transfusion} & C+L & 68.9 & 71.7 & 87.1 & 60.0 & 68.3 & 60.8 & 33.1 & 88.4 & 73.6 & 52.9 & 86.7 & 78.1\\
\textbf{\model} (Ours) & C+L & \textbf{70.2} & \textbf{72.9} & \textbf{88.6} & 60.1 & \textbf{69.8} & \textbf{63.8} & \textbf{39.3} & 89.2 & 74.1 & 51.0 & 86.5 & \textbf{80.0}\\\bottomrule 
\end{tabular}
\end{table*}

==> visuals/results/joint.tex <==
\begin{wraptable}{r}{5.2cm}
\centering\small
\vspace{-15pt}
\caption{Joint detection and segmentation training (trained for 10 epochs).}
\vspace{-5pt}
\label{tab:results:analysis:joint}
\setlength{\tabcolsep}{3pt}
\scalebox{0.85}{
\begin{tabular}{lccc}
\toprule
& NDS & mIoU \\
\midrule
Detection only & 70.4 & -- \\
Segmentation only & -- & 58.5 \\
\midrule
Joint (\textit{shared BEV encoders}) & 69.7 & 54.0  \\
Joint (\textit{separate BEV encoders}) & \textbf{69.9} & \textbf{58.4} \\
\bottomrule 
\end{tabular}
}
\vspace{-10pt}
\end{wraptable}

==> visuals/results/sparse_lidar.tex <==
\begin{table*}[t]
\caption{\model consistently outperforms all existing sensor fusion methods in sparse LiDAR 3D object detection on the nuScenes \texttt{val} split. It achieves up to \textbf{20.2} mAP improvement over MVP in the challenging 1-beam LiDAR setting.}
\label{tab:results:detection:sparselidar}
\setlength{\tabcolsep}{2.5pt}
\small\centering 
\begin{tabular}{lcccccccccc} \toprule[1pt]
& Modality & mAP & NDS & mATE & mASE & mAOE & mAVE & mAAE & MACs (G) & Latency (ms)         \\\midrule[1pt]
\textbf{1 beam LiDAR} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \midrule[0.5pt]
CenterPoint~\cite{yin2021center}     & L  & 12.3 & 35.8 & 57.2 & 29.3 & 59.6 & 41.1 & \textbf{16.0} & 61.2 & 55.4\\
PointPainting~\cite{vora2020pointpainting}         & C+L & 21.7 & 39.8 & 54.0 & 29.1 & 64.8 & 42.7 & 20.7 & 278.1 & 159.9\\
MVP~\cite{yin2021multimodal}    & C+L & 22.6 & 39.8 & 54.5 & 28.7 & 68.4 & 42.1 & 21.2 & 278.5 & 162.4\\
FUTR3D~\cite{chen2022futr3d}    &  C+L & 41.3 & 50.0 & 61.0 & \textbf{26.9} & \textbf{40.8} & 59.0 & 18.7 & -- & --\\
\textbf{\model} (Ours)    &   C+L & \textbf{42.8} & \textbf{52.0} & \textbf{49.4} & \textbf{26.7} & 42.9 & 53.7 & 20.9 & 172.0 & 107.0\\\midrule[1pt]   
\textbf{4 beam LiDAR} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \midrule[0.5pt]
CenterPoint~\cite{yin2021center}     & L  & 40.9 & 54.9 & 36.2 & 27.5 & 40.7 & 32.8 & \textbf{17.7} & 68.5 & 57.5\\
PointPainting~\cite{vora2020pointpainting}         & C+L & 52.1 & 60.2 & 36.4 & 27.0 & 44.6 & 31.9 & 19.1 & 285.2 & 162.5\\
MVP~\cite{yin2021multimodal}    & C+L & 54.2 & 61.4 & 34.7 & 27.0 & 44.6 & 30.8 & 20.0 & 285.9 & 165.1\\
FUTR3D~\cite{chen2022futr3d}    &  C+L & 54.9 & 61.5 & 41.1 & 26.3 & \textbf{33.6} & 35.0 & 18.6 & -- & --\\
\textbf{\model} (Ours)    &   C+L & \textbf{55.7} & \textbf{63.2} & \textbf{33.9} & \textbf{26.2} & 38.8 & \textbf{28.3} & 19.6 & 179.3 & 109.4\\\midrule[1pt]   
\textbf{16 beam LiDAR} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \midrule[0.5pt]
CenterPoint~\cite{yin2021center}     & L  & 46.3 & 58.5 & 35.3 & 26.2 & \textbf{36.0} & 31.1 & \textbf{18.3} & 75.3 & 61.4\\
PointPainting~\cite{vora2020pointpainting}         & C+L & 56.3 & 63.2 & 34.0 & 26.5 & 41.4 & 29.1 & 19.1 & 291.9 & 166.3\\
MVP~\cite{yin2021multimodal}    & C+L & 57.9 & 63.8 & 33.9 & 26.4 & 41.2 & 29.7 & 20.4 & 292.7 & 167.1\\
FUTR3D~\cite{chen2022futr3d}    &  C+L & 57.7 & 63.4 & -- & -- & -- & -- & -- & -- & --\\
\textbf{\model} (Ours)    &   C+L & \textbf{58.0} & \textbf{64.4} & \textbf{32.5} & \textbf{26.1} & 39.7 & \textbf{28.6} & 19.1 & 186.1 & 113.8\\\bottomrule[1pt]  
\end{tabular}
\end{table*}

==> visuals/results/stability_detection.tex <==
\begin{table*}[t]
\caption{\model achieves stable results on the \texttt{val} split of the nuScenes dataset.} %Here, C.V., Ped., Motor., Cone are the abbreviations for construction vehicles, pedestrians, motorcyclists and traffic cones.}
\label{tab:results:stability}

\begin{subtable}[t]{\linewidth}
\small\centering 
\setlength{\tabcolsep}{6.5pt}
\caption{Metric breakdown for 3D object detection}
\label{tab:results:stability:detection:metric}
\begin{tabular}{ccccccc} \toprule
 mAP ($\uparrow$) & NDS ($\uparrow$) & mATE ($\downarrow$) & mASE ($\downarrow$) & mAOE ($\downarrow$) & mAVE ($\downarrow$) & mAAE ($\downarrow$) \\\midrule
68.52 \textsubscript{($\pm$0.03)} & 71.36 \textsubscript{($\pm$0.08)} & 28.85 \textsubscript{($\pm$0.15)} & 25.41 \textsubscript{($\pm$0.06)} & 30.53 \textsubscript{($\pm$0.90)} & 25.48 \textsubscript{($\pm$0.31)} & 18.73 \textsubscript{($\pm$0.08)}\\\bottomrule  
\end{tabular}
\end{subtable}
~
\begin{subtable}[t]{\linewidth}
\small\centering 
\setlength{\tabcolsep}{1.0pt}
\vspace{5pt}
\caption{Per-class result breakdown for 3D object detection}
\label{tab:results:stability:detection:class}
\scalebox{0.95}{
\begin{tabular}{cccccccccccc} \toprule
 mAP & Car & Truck & Bus & Trailer & C.V. & Ped. & Motor. & Bike & Cone & Barrier\\\midrule
68.5 \textsubscript{($\pm$0.0)} & 89.3 \textsubscript{($\pm$0.0)} & 65.3 \textsubscript{($\pm$0.5)} & 75.4 \textsubscript{($\pm$0.4)} & 43.2 \textsubscript{($\pm$0.5)} & 29.7 \textsubscript{($\pm$0.5)} & 88.2 \textsubscript{($\pm$0.1)} & 78.5 \textsubscript{($\pm$0.3)} & 64.5 \textsubscript{($\pm$0.4)} & 79.5 \textsubscript{($\pm$0.4)} & 71.6 \textsubscript{($\pm$0.5)} \\\bottomrule  
\end{tabular}
}
\end{subtable}
~
\begin{subtable}[t]{\linewidth}
\small\centering 
\setlength{\tabcolsep}{6.5pt}
\vspace{5pt}
\caption{Per-class result breakdown for BEV map segmentation}
\label{tab:results:stability:segmentation:class}
\begin{tabular}{cccccccc} \toprule
 mIoU & Drivable & Ped. Cross. & Walkway & Stop Line & Carpark & Divider \\\midrule
62.49 \textsubscript{($\pm$0.20)} & 85.40 \textsubscript{($\pm$0.06)} & 60.59 \textsubscript{($\pm$0.26)} & 67.35 \textsubscript{($\pm$0.20)} & 51.36 \textsubscript{($\pm$0.51)} & 56.50 \textsubscript{($\pm$0.42)} & 53.75 \textsubscript{($\pm$0.08)}\\\bottomrule  
\end{tabular}
\end{subtable}
\end{table*}




==> visuals/results/visualization.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/results/visualization.pdf}
    \caption{Qualitative results of BEVFusion on 3D object detection and BEV map segmentation. It accurately recognizes distant and small objects (top) and parses crowded nighttime scenes (bottom).}
    \label{fig:results:visualization}
\vspace{-15pt}
\end{figure*}
